The Software Genome Project: Venture to the Genomic Pathways of Open Source Software and Its Applications

With the boom in modern software development, open-source software has become an integral part of various industries, driving progress in computer science. However, the immense complexity and diversity of the open-source ecosystem also pose a series of challenges, including issues of quality, security, management, maintenance, compliance, and sustainability. Existing open-source governance approaches, while excelling in community building and collaboration, still face shortcomings in decentralized management, security, and maintenance. To address these challenges, inspired by the Human Genome Project, we treat the software source code as software DNA and propose the \textbf{Software Genome Project}, which is geared towards the secure monitoring and exploitation of open-source software. By identifying and labeling integrated and classified code features at a fine-grained level, and effectively identifying safeguards for functional implementations and non-functional requirements at different levels of granularity, Software Genome Project builds a complete set of software genome maps to help developers and managers gain a deeper understanding of software complexity and diversity. By dissecting and summarizing functional and undesirable genes, Software Genome Project helps facilitate targeted software remediation and optimization, provides valuable insight and understanding of the entire software ecosystem, and supports critical development tasks such as technology selection and open source governance. This project is expected to drive the evolution of software development towards more efficient, reliable, and sustainable software solutions.

==> outline/framework.tex <==
\section{Software Genome Project}

Our project is to develop a unified framework to conduct open-source software intelligence analysis from the perspective of biological DNA. 
This initiative focuses on leveraging the maturity of biological genes to build more standardized open-source rules to meet real-world challenges, while protecting open-source security. 
As shown in Figure \ref{fig:sgp}, our project consists of \emph{Software Genome Construction and Annotation}, \emph{Software Intelligence Genome Construction and Annotation}, \emph{Software Genome Analysis}, \emph{Software Composition Analysis}, \emph{Software Maintenance}, and \emph{Open Source Governance} to enhance the security, resilience, and reliability of open-source software in the physical world. 
 
\subsection{Software Genome Construction and Annotation}
This phase aims to lay the foundation for creating the world's inaugural software genome and, subsequently, to employ it as the basis for crafting an innovative software gene repository. 

\subsubsection{Sample Collection → Software Code Collection.}
Given the excessive amount of software repositories in real world, it is crucial to fully examine the consistency of all software within reasonable complexity and resource consuming. 
In this task, we aim to propose a systematic solution on the efficient collection of the most valuable repositories from the perspective of constructing software genome. 
Therefore, we initialize the construction of software genome by sorting out the most recognized software repositories. 
Considering that most existing research on software repository mining have proposed various criteria on selecting representative repositories for experiment and analysis. W
e first revisit these papers to identify the mostly recognized metrics on selecting representative repositories, such as stars, forks, issues, commits and contributors, etc. 
Specifically, we investigate both their representativeness of important software repositories and availability from the aspect of ecosystem-wide acquisition, so that they can be properly acquired or calculated for large scale analysis.
Based on these, we interpret their distribution in the entire open-source ecosystem and set the threshold as a coarse-grained bar to sort out the most recognized repositories as the initial candidate projects. 
Specifically, as most open-source repositories are with limited value (\ie not well organized and maintained), we aim to set the threshold as a relatively low bar to exclude meaningless repositories based on distribution analysis. 


\subsubsection{DNA Sequencing → Software Scope Determination}
Next, we intercept the source code of each selected repository to identify the features of software brought by individual code fragments. Specifically, from the perspective of diversity of genome, we value a software repository by its contribution of code diversity to the ecosystem. Theoretically, a repository with more unique and representative code fragments tends to have contributed more value than repositories that are mostly copied from others and have less unique code fragments. Therefore, based on the selected candidate repositories, we first calculate their function-level value by accumulating their uniqueness. Specifically, for a function itself, its value is usually defined by its complexity, and existing work has defined the quantitative calculation its value by:
$$
Value\left(f\right)\ =\ 171\ -\ 5.2\ \cdot\ {ln}ln\ \left(HV\right)\ \ -\ 0.23\ \cdot\ \left(CC\right)\ -\ 16.2\ \cdot\ {ln}ln\ \left(LOC\right)\ 
$$
Where HV stands for Halstead Volume, CC denotes Cyclomatic Complexity, LOC denotes Lines of Code. However, when considering the contribution of code diversity to the ecosystem, such value could be compromised it many duplicates can be found in different repositories. Therefore, before aggregating the overall contribution of repositories, we split the contribution value of each function by the duplications so that these repositories can share the contribution. Moreover, we also exclude the value of commonly used functions due to too massive usage to preserve code intelligence. The final repository contributions can be calculated as:
$$
contribution\left(repo\right)=\left(\sum_{f\in r e p o}\frac{value\left(f\right)}{frequency\left(f\right)}\right)\cdot\frac{unique\_func_count}{all\_func_count}
$$
Based on these, we can identify all the functions that represent the most code diversity in the ecosystem, which constructs the majority of software genome.

\subsubsection{Sequence Assembly → Software Repository Closure}
Although task 1.1 sorts out the most recognized repositories as the objects to retrieve software genome, there could be still plenty of software repositories missed due to poor performance on specific criteria on selecting repositories. Therefore, we plan to introduce a bi-directional approach to incrementally expanding the software genome by including more representative repositories, and meanwhile, excluding outlier repositories that have less value while acts well on the basic criteria. However, considering that most repositories could be filtered out by our criteria, it could be resource-wasting if simply traversing these repositories without prioritization, which may delay the closure of software genome construction. Therefore, in this task, we aim to propose an algorithm to prioritize the incrementally add back repositories that are initially excluded, with which, we can proceed to the closure of software genome with processing relatively minimal number of software repositories.
We first sort out repositories that tend to be more recognized and sorting them in batches to supplement the feature dataset constructed in task 1.2. Specifically, each repository can be represented by a vector of selected metrics in task 1.1. Based on this, we plan to use Local Outliers Factor (LOF) to detect the potentially mis-filtered projects. 
For repositories that are clear outliers, we believe they are more likely to have outstanding values compared with the majority of repositories that perform poor in all these metrics. 
Specifically, for a collection of repositories that are filtered out, we sort them by LOF and examine them as batches to supplement the feature dataset, until the feature dataset stops to expand with reasonable cost-effectiveness.

\subsubsection{Structural Annotation → Software IP Analysis.}
After obtaining the feature dataset, we employ multifaceted analyses to understand the structural properties and identify key ``software genes''. 
We first construct a call graph to represent the complex caller-callee relationships between all functions. 
%The graph is a visual representation of software processes and connections. 
Next, we conduct advanced social network centrality analysis (\eg degree centrality and closeness centrality) to identify key nodes (similar to``influencer'') that control the behaviour and information flow of the software.
Apart from analyzing the connections between functions, we also perform a comprehensive code analysis for each function to reveal the code complexity.
Combining these local (\ie code complexity) and global (\ie centrality) insights, we create a ranking for all functions, highlighting their relative importance and contribution to the software ecosystem. 
This procedure blends complex analyses ranging from call graph construction to centrality assessment and code complexity assessment, culminating in a robust software gene pool that captures the genetic nature of software.


\subsubsection{Functional Annotation → IP Functionality Analysis.}
In this process, we'd like to assess the functionality of software genes derived from the previous step.
We closely examine the code's structure, variables, and other program details to glean insights into its intended purpose.
We also explore any accompanying comments  provided by developers during the code's creation, which can often offer invaluable insights into the code's intended functionality.
Moreover, if available, we will execute the code segment in a controlled environment by using some testing cases to verify that the code behaves as intended and produces the expected results. 
Our purpose is to answer fundamental questions about what the code achieves, how it accomplishes its goals, and the specific problem it addresses.
Once we have a solid understanding of the code's functionality, we proceed to provide essential code details for accurate documentation.
This document will serve as the dictionary of our ``software genes''.


\subsection{Software Intelligence Genome Construction and Annotation}
In this phase, we aim to amass the most extensive software defective gene repository and we call it software intelligence genome.
It includes a comprehensive range of software issues such as vulnerability, malicious code, and sensitive code. 
%Moreover, for each collected source code, we conduct corresponding detailed analysis to retrieve the code functionality, which can contribute to the advancement of software reliability and security practices. 

\subsubsection{Inheritable Disease Gene Collection → Vulnerability Collection}

Collecting software vulnerability data is essential for effective risk management, informed decision-making, and maintaining the security of software systems. 
This data enables organizations to prioritize and apply security patches, mitigate potential risks, ensure regulatory compliance, and enhance incident response strategies. 
It empowers security teams with threat intelligence, aids in vendor assessment, supports security training efforts, and fosters a culture of continuous improvement. 
Organizations can proactively protect against emerging threats by analyzing vulnerability data, making strategic software choices, and demonstrating their commitment to robust cybersecurity practices. 
Our overarching aim is to establish a comprehensive data platform housing curated, current, and high-caliber vulnerability data. 
This data reservoir will serve as the foundation for the creation of a secure package manager and an online alarm system, enabling enhanced software security measures.

\emph{Evaluation of Vulnerability Data Quality from Mainstream Sources.}
In the practical realm, a significant portion of vulnerability data originates from online databases such as CVE and NVD, each hosted by distinct entities with specific objectives. For instance, NVD, overseen by the U.S. government, strives to comprehensively document the landscape of existing vulnerabilities, whereas OSV, sponsored by Google, focuses exclusively on vulnerabilities present in widely utilized open-source libraries.
Our objective is to examine each source of vulnerability data and assess its quality. To achieve this, we will establish a robust data pipeline to aggregate vulnerability data from diverse sources, implementing an incremental update approach to ensure the continuous accuracy of the data. Furthermore, we will develop a data dependency analysis framework to elucidate the provenance of the data and effectively eliminate any redundancies. Through attribution of individual vulnerability facets, we will undertake differential analyses to discern disparities in the portrayal of identical vulnerabilities.

\emph{Vulnerability Quality Improvement via Programming Analysis and Large Language Model.}
The vulnerability information procured from online sources may exhibit inaccuracies or omissions. Our objective is to harness advanced programming analysis techniques in conjunction with the capabilities of a large language model (LLM) to enhance the information. A case in point pertains to the established methodologies for ascertaining the scope of vulnerability impact, often reliant on human auditing, a process susceptible to errors. We intend to extrapolate this scope directly from the code lines. In the case of each CVE entry, we will perform an execution trace traversal of functions using program slicing techniques, outlining vulnerability constraints through symbolic execution. Subsequently, we will employ fuzzy matching techniques to align these constraints with susceptible lines of code, enabling rapid and precise identification of the vulnerability's presence within any given software iteration. Furthermore, we will train the language model to comprehend source code commits, thus enabling it to predict accurate commit messages and vulnerability descriptions. 

This endeavor will significantly refine critical facets of vulnerability information, encompassing the scope of impact, patch information, and proof of concept (PoC) elucidations. All the downstream tasks such as vulnerability prediction, patch generation, and PoC detection will benefit from the improvement of the data quality.

\subsubsection{Inheritable Disease Gene Collection → Malicious Code Collection}

Malicious code severely threatens software ecosystems through viruses, worms, spyware. It steals data, hijacks systems, causes financial and reputation damage. Research into malicious code is crucial to analyse evolving techniques, develop detection methods, and strengthen defence.
Our objective is to create a comprehensive dataset of malicious code, encompassing source code and binary files across various programming languages, including Python, C, and Java. This diverse dataset enhances our understanding of malicious code's structure and behavior, offering a robust foundation for software genomics research. To ensure broad coverage, we will collect data from multiple channels, including underground forums, community platforms, and databases like VirusShare and VX Heaven. Additionally, we'll explore GitHub to include diverse source code samples, expanding the dataset's scope.

In collection process, we tailored strategies to the unique attributes of different sources. Web crawling modules were developed for underground forums and community platforms, automatically retrieving malicious code-related posts and attachments using predefined keywords. Source code and attachments were extracted, downloaded, and stored from these posts. For malicious code databases like VirusShare, VX Heaven, VirusSign, and Malshare, we utilized API interfaces to access data through queries, including vital metadata and hash values. We also designed data collecting modules for GitHub, targeting diverse programming languages. These modules independently searched and downloaded relevant source code repositories. Ensuring data quality, we employed hash algorithms for deduplication and conducted integrity checks. The resulting dataset was annotated and categorized, detailing its origin, timestamp, and malicious code family. Through this thorough process, we aim to provide a high-quality, diverse malicious code dataset for future research.


\subsubsection{Inheritable Disease Gene Collection → Sensitive Code Collection}

The open-source software ecosystem thrives on the principle of collaboration and shared knowledge, while such openness can inadvertently become a conduit for the dissemination of sensitive or harmful content. Considering the diversity of, i.e., cultural, ethical, and legal backgrounds of developers, contributors, and users, sometimes some sensitive code in open-source repositories could lead to clashes, misunderstandings, and misuse. The absence of a comprehensive framework to govern sensitive content undermines the safety, inclusivity, and ethical use of open-source software. There is a pressing need to establish clear guidelines and mechanisms to identify, manage, and mitigate sensitive content, ensuring that open source remains a positive, productive, and safe environment for all stakeholders. Addressing this issue is not just a matter of ethical responsibility but is crucial for sustaining the integrity and public trust in the open-source ecosystem.

Therefore, our objective is to collect and create comprehensive dataset of sensitive code in open-source repositories. Specifically, there are three different types of sensitive code we plan to collect. First, user-sensitive code: developers, especially new contributors of open-source repositories could accidentally commit their sensitive information into open repositories, such as private information, access tokens, and access of private databases, while these sensitive codes could be dangerous if they are utilized by malicious attackers. Next, behaviour- sensitive code: some open-source components could pose security risks due to the special system privileges they require. Even though these components are not malicious, attackers can exploit these privileges when the components are incorporated into broader systems, leading to unauthorized access or other security breaches. Moreover, politics-sensitive code: Given the global and diverse nature of contributors and users, open-source repositories can become arenas where political biases, propaganda, or sensitive information are disseminated, either inadvertently or deliberately. The need to monitor and manage these repositories for political sensitivities is paramount, not only to maintain the integrity and neutrality of the projects but also to prevent potential legal and ethical violations. Vigilance in this domain ensures that open-source platforms remain inclusive, respectful, and focused on technological advancement, unmarred by divisive or sensitive political issues. 

Collecting and monitoring these sensitive codes could benefit the proper detection and governance of open-source ecosystems, and analysing these sensitive codes could also strengthen the understandings of sensitive information existing in open-source repositories and promoting the detection of sensitive code from user aspect.


\subsubsection{Annotation → Code Functionality Analysis}

Conducting functional annotation for vulnerabilities, malicious code, and sensitive code involves thoroughly documenting their behaviors, potential impacts, and the context in which they can be exploited or pose risks.

As for vulnerabilities functionality analysis, we begin by understanding the nature of the vulnerability. This includes identifying the specific type (e.g., SQL injection, cross-site scripting) and how it affects the software. Determine how it can be triggered and what it may lead to in terms of unauthorized access, data breaches, or system compromises. We’d like to annotate the context in which the vulnerability can be exploited, describe the impact on the software, such as the potential consequences of exploitation, and any relevant risk factors. Moreover, we will analyze potential scenarios where the vulnerability might be exploited, including attack vectors, attacker profiles, and the methods they might employ. This helps in assessing real-world risks.

As for malicious code functionality analysis, we begin by understanding the behavior of the malicious code, such as its purpose (e.g., data exfiltration, system disruption) and how it operates within the software. Then, we will document its specific actions, payloads, and describe the conditions under which the malicious code is triggered or executed. This includes events, user actions, or system states that activate the malicious behavior. Also, we will document the payload carried by the malicious code, if applicable, and specify the types of malicious files, commands, or data manipulations it performs. If the malicious code can propagate within the software or to other systems, detail how this occurs. Include information on communication protocols or vectors used for spreading.

As for sensitive code functionality analysis, we begin by identifying code segments that handle sensitive data, such as user credentials, personal information, or financial data. Be explicit about where this code is located and describe how the sensitive data is processed within the code. This includes data collection, storage, transmission, and disposal practices. In addition, we will document the access control mechanisms in place for sensitive data and detail who has permissions to interact with this data and under what conditions. Meanwhile, we consider any industry-specific compliance requirements (e.g., GDPR, HIPAA) or security standards that the code must adhere to, and annotate how the code complies with them.

By conducting functional annotation for vulnerabilities, malicious code, and sensitive code, we can provide essential documentation to guide developers, security experts, and users in understanding and addressing potential risks and security issues.


\subsection{Software Genome Analysis}
The objective of this WP is to perform in-depth analysis on our collected genomics, including gene-gene interactions analysis, gene family classification, gene phenotype analysis, and gene evolution analysis. They enable us to draw connections between individual genes, identify shared functionalities, and recognize dependencies that contribute to the software's overall functionality, quality, and evolution.

\subsubsection{Gen-gene Interactions Analysis → Software Dependency Analysis}

Abundant evidence and accumulated experience show that the traits of certain complex diseases are collectively influenced by interactions among multiple genes. Consequently, investigating the interplay between genes from a biological perspective holds substantial value. In pursuit of comprehensive open-source intelligence analysis, we also extend our examination to the interactions among software genes, analogous to the dependencies within genes. Our analysis encompasses not only the directly defined software dependencies within package managers but also delves into more intricate relationships induced by code cloning. 

\emph{Package Manager-based (PM-based) Dependency Analysis.}
PM-based dependencies entail the explicit relationships established within the codebase to ensure the availability and compatibility of external libraries or components. These dependencies are meticulously defined within the package management system, enabling developers to easily integrate and utilize external resources. This type of dependency encompasses a structured approach where software modules rely on the functionality provided by external packages. The package manager handles the retrieval, installation, and version management of these dependencies, ensuring a controlled and organized integration process. Developers can explicitly specify the required version of a package, enabling precise control over the software's behavior and compatibility with other components. To extract PM-based dependencies from a software project, we will follow these steps: 1) Analyze Package Files: Identify the package management files used in the project, such as package.json for JavaScript projects, requirements.txt for Python, or pom.xml for Java. These files list the external packages required by the project. 2) Parse Dependency Definitions: Extract the package names and versions specified in the package files. These definitions indicate the required external components and their compatibility criteria. 3) Retrieve Metadata: Utilize the package manager's API or repository to retrieve metadata about each dependency, including its version, dependencies, and other relevant information. 4) Build Dependency Graph: Construct a dependency graph by connecting the project's modules or components to their corresponding external packages. Include information about version constraints and compatibility. 5) Analyze Interactions: Analyze how the dependencies interact within the codebase. This involves identifying where and how the external packages are utilized, and how they contribute to the software's functionality.

\emph{Code Clone-based (CC-based) Dependency Analysis.}
CC-based dependencies stem from the reuse of existing code fragments or patterns within the software. This form of dependency emerges when portions of code are duplicated across different parts of the software, often to replicate a specific functionality or design approach. While not explicitly indicated as dependencies within the codebase, these cloned code segments inherently create interconnections among various sections of the software. To extract CC-based dependencies from a software project, we will follow these steps: 1) Identify Cloned Fragments: Design novel code analysis tools to identify duplicated code fragments within the project. These tools can detect similar or identical code patterns across different parts of the codebase. 2) Trace Clones: Trace the instances of cloned code to understand where they are duplicated and how they are utilized across the software. 3) Analyze Impact: Analyze the impact of code changes in one cloned instance on other instances to understand how changes propagate through the codebase due to these clones. 4) Quantify Relationships: Quantify the relationships between cloned code fragments and identify shared functionalities, data structures, and patterns that contribute to software behavior. 5) Visualize Dependencies: Create visualizations or graphs that illustrate the connections between different cloned instances. This can help developers understand the intricate relationships and identify potential areas for optimization.

Both types of dependencies contribute to the overall structure and behavior of the software. Package manager-based dependencies provide controlled integration with external resources, enhancing modularity and code reusability. Code clone-based dependencies, while not as overt, underscore the importance of code organization and shared patterns within the software. By considering both forms of dependency, a comprehensive view of the software's interconnectedness emerges, enabling developers to optimize performance, mitigate risks, and enhance software quality.

\subsubsection{Family Classification → Software Clustering}

The excessive adoption of open-source artifacts in modern software development has promoted the prosperity of open-source ecosystems, including both the published third-party libraries and code snippets that are widely reused by developers (i.e., software genes). With this, users can bypass the need to code from scratch and accomplish more complex and challenging tasks in easier ways. However, the vast and complex ecosystem of open-source artifacts make it difficult to properly comb the vast knowledge and coding practices, which makes it insufficient to reuse existing artifacts to accelerate modern software development (i.e., guiding LLMs for SE). In this case, we aim to dive into the applications of software genes and comb their usage practices and diversity in different domains.
Our objective is to construct a comprehensive map ton figure out the ability and diversity of software genes, including the classifications of software genes, their scope and applicable domains, usage practices, possible combinations, and their evolutions. Specifically, due to the diversity of software genes, they could be with different size and formats, we aim to dig out the possible combination of software genes in a mixed solution.

\emph{Software Gene Clustering.}
First, the construction of software genome has unveiled the existence of software genes in different software repositories, including both open-source applications and third-party libraries, and we are able to utilize such existence to cluster software genes by the domains of applications and third-party libraries. Specifically, we plan to use two types of information to grouping software genes. 1) Co-existence. Software genes could be integrated into applications or third-party libraries within similar domains. In this case, we investigate the co-existence of software genes in open-source artifacts. If such co-existence is with high possibility, it may indicate that these software genes are usually used in software within similar domains. 2) Dependency Relationship. As the most important part of open-source ecosystems, third-party libraries play important roles in software development, which also provide significant portion of software genes. Therefore, we trace the dependency relationships among third party libraries with abundant genes. Considering that dependency relationships naturally indicate the connection between software artifacts, software genes that are within third-party libraries on the same dependency paths should also naturally have implicit dependencies in specific domains. Therefore, we aim to combine this information as the distance factor to classify software genes to different domains.

\emph{Software Gene Semantics.}
After clustering these software genes, we aim to comb these clustered software genes and identify the semantics of them. Specifically, we identify the correlation of software genes by mining the frequent patterns appearing in existing software, based on which, we aggregate these genes to identify their usage and semantics by integrating LLM techniques. Moreover, with the classification of software domains, we can interpret software genes with their usage and presentations on software functionalities. Furthermore, based on their usage, the critical genes for different software domains can be also identified, such as the common practices and fundamental software genes, which could be further utilized to guide future software development to improve efficiency.


\subsubsection{Phenotype Analysis → Software Portrait}

Apart from the defective software genes we identified, there are more generalized software defects hidden in the commonly used third party software artifacts, such as code smells, poor maintainability, potential low code quality, etc. Although these software defects do not directly affect the regular functionality of software, they could still introduce potential threats to the long-terms maintenance of software. Therefore, it is still of great importance to properly identify these software defects and take countermeasures to enhance the long run of software.
The objective of this task is to summarize these kinds of software defects in a comprehensive way, including not only factors of different dimensions on software assurance, but also proper and measurable metrics to appropriately reflect these factors to build up the profile for software genes. Besides the taxonomy, we also aim to propose a set of tool chains to properly identify and measure them in a well-organized way, and aggregate these measurement to standardized metrics.

\emph{Software Assessment Taxonomy.}
First, we review existing academic papers and related tools from both academic and industrial, and retrieve the factors that currently researchers and developers care during their development. Specifically, we conclude the taxonomy of software defects from the following dimensions: 1) Software Quality, including the wrong and bad code smells in software which could lead to software defects during runtime; 2) Software Security, denoting the potential security threats identified as defects in software; 3) OSS compositions, representing the potential threats introduced by reused third-party artifacts, such as libraries and code snippets; 4) Maintainability, reflecting the maintenance of software components in different repositories, for instance, software genes from inactive repositories tend to have poor maintenance when issues happen; 5) Business Risk, annotating the commercial risks of software due to license and copyright issues hidden in reused third party artifacts. Based on these coarse-grained classifications, we aim to propose a comprehensive taxonomy to summarize these various software defects.

\emph{Software Defect Measurement.}
With the support of fine-grained taxonomy of software defects, we then develop the tool chains to properly measure these factors in comprehensive ways. Considering that not all factors can be perfectly detected by existing tools, we propose a combination strategy that aggregates the detection outcomes of different tools to reflect the performance of software genes on different dimensions. Specifically, different weights should be granted for different defects detected by these tools, for example, vulnerabilities should be more weighted that code smells as they bring more severe consequences and could be more probably to be utilized. 


\subsubsection{Evolution Analysis → Software Evolution Analysis}

Software genes are also dynamically evolving along with time, like biological genes. Analysing the evolution of the open-source ecosystem is crucial to comprehend its growth, dynamics, and adaptive behaviours. As open source communities expand, they could encounter various influences, including technological innovations and diverse contributors. A concise analysis yields essential insights into trends, challenges, and opportunities, forming the basis for strategic decision-making and policy development. Such studies are vital in enhancing the quality, security, and inclusivity of open-source software, ensuring its sustained impact on the global technological domain.

Therefore, this task aims to surveillance the dynamic changes of software genes in open-source ecosystems to identify the forms, reasons, and trends of software changes during evolution. In this case, we aim to identify how software development changes during evolution and conclude the practice changes during software development. For instance, the commonly used coding practices could be replaced when new technologies appear. First, for fundamental software genes, we monitor and analyse the changes of how developers incorporate existing software genes, including the addition, removal, and replacement of software genes, to achieve different requirements, and these practices could benefit the future composition when conducting automated software development. Next, for domain specific genes, we also monitor how these genes are introduced from other domains and how genes communicate among different domains, which could help the conclusion of technical stacks and guide further component selections when designing new software. Moreover, it is also crucial to keep monitoring the growth and decline of supports for different domains in open-source ecosystems, for example, when techniques are threatened by poor maintenance, more resources and efforts could be guided by the community to ensure the sustainability of critical infrastructures. Based on these, we can timely predict the evolution of techniques in software development and raise up proper recommendations accordingly.



\subsection{Software Composition Analysis}
The objective of this WP is to translate the insights gained from our software genome analysis into practical real-world applications. Leveraging our understanding of software genomes, we model genetic testing and develop predictive models to enhance software composition analysis (SCA) from four different perspectives (i.e., component analysis, clone detection, dependency analysis, and vulnerability analysis). 

\subsubsection{Newborn Screening → SCA-Component Analysis}

After previous processing, we can build a well-organized and extensive dataset (i.e, software genomics) of known software genes which encompasses various programming languages, frameworks, and libraries. This dataset is akin to having a reference library of genetic information for comparison. In the context of software genomics, newborn screening translates to pinpointing the source code of the new software project that requires screening. This entails collecting and isolating the code from the rest of the project, akin to isolating specific genetic material for analysis.

In this pivotal stage of software composition analysis, the code of the new software project is meticulously compared to our collected software genomics. This comparison process involves several key elements. First, we design some advanced pattern recognition techniques to identify specific code structures, naming conventions, and other structural characteristics that align with those in our collected software genomics. Think of this as recognizing genetic markers or sequences that match known patterns in a biological sample. Then, we conduct semantic analysis to understand the functional aspects of the code. This involves assessing how the code segments in the new project perform similar functions to those in our collected software genomics. Next, to ensure accuracy, we compare not only the code structure but also the versioning information. This is crucial for identifying whether the code segments in the new project correspond to specific versions of known software genes. After ensuring the version, we use some probabilistic matching algorithms to calculate the likelihood of a code segment in the new project being a match to a known gene. This helps in minimizing false positives and enhancing the precision of identification. 

Once we identify matches or similarities between the code in the new project and our collected software genomics, the process moves on to code segment extraction. This is a meticulous process that involves segment Isolation and code preservation. As for segment isolation, the segments of code that match known software gene are isolated from the larger codebase of the new project. This ensures that only the relevant genetic components are extracted, similar to how specific genetic information is extracted from a biological sample. While the segments are extracted, the integrity of the code is preserved. This ensures that the extracted components maintain their functionality and can seamlessly integrate into the broader software ecosystem. It's akin to preserving the biological information extracted from a sample for further study or application. The extraction of software genes is not limited to the code itself, it also encompasses the collection of essential metadata including component information and license information. Details such as the component's name, version, and description are meticulously recorded. This is akin to creating a detailed genetic profile that includes genetic markers, familial history, and observed traits. Licensing details are also noted to ensure compliance and proper usage. This is similar to understanding the legal aspects of genetic information, such as patents and rights.

By conducting these detailed processes of comparison, code segment extraction, and metadata collection, we ensure not only the precise identification of software components but also the preservation of their functional integrity and the comprehensive documentation of their characteristics. This meticulous approach paves the way for seamless integration into software ecosystem and future software development and maintenance efforts.

\subsubsection{Paternity Testing → SCA-Clone Detection}

In the context of treating software source code as genes and utilizing a software genomics framework, conducting "Paternity Testing" can be likened to code clone detection. Code clone detection helps identify instances where segments of code within a project share a common ancestry or source, which is akin to establishing paternity or parentage in a biological context.

In this task, we design some novel code clone detection techniques which can scale to billion lines of code analysis. Our tool consists of two parts: Token-based Filtering and Tree-based Verification. During the Token-based Filtering phase, we first extract all functions from the source files and concatenate all the adjacent N lines of code for each function. In this way, the inverted index can be created for locating. Then, we adopt the filter similarity calculation formula mainly based on the number of shared N-Lines as the first filter. After that, we compute the token similarity of the remaining pairs based on their token sequences as the second filter. During Tree-based Verification phase, two techniques based on AST are adopted in our work. The first technique is to use a subtree matching algorithm based on hash trees to detect clones while the other is to analyze the tree vectors for clone detection. We use the above two methods to verify the token-filtered pairs separately, and finally combine their results to report our detected clone pairs. This tool will be used to measure the similarity scores of two code snippets. 

Similarity scores are compared against a predefined threshold. High similarity scores suggest a strong likelihood of code clones. Additionally, probabilities may be calculated to estimate the likelihood of code segments sharing a common origin, similar to establishing probabilities in genetic testing. Code segments that surpass the threshold are confirmed as code clones. These are instances where the code exhibits substantial commonality, much like confirming paternity when genetic markers closely match. Code clones are categorized based on the level of similarity and variations. This categorization provides insights into the heritage of the code and the extent of shared ancestry, similar to classifying genetic relationships. Each identified code clone is associated with metadata, including the location of code clones, their respective origins (source files or repositories), metadata about the authors or teams involved, and information regarding the extent of similarity. This documentation serves as a reference for code maintenance, audits, and future development, similar to maintaining comprehensive records of genetic testing results for reference in medical genetics.

By executing these detailed steps within our "Paternity Testing" for code clone detection, we can systematically identify, assess, categorize, and document code clones within our software genomics framework. This rigorous approach ensures that code quality and maintainability are upheld and contributes to a deeper understanding of the code's shared heritage and ancestry.


\subsubsection{Genetic Traceability → SCA-Dependency Analysis}

"Genetic Traceability" through dependency analysis can be compared to tracing genetic lineage and inheritance. Through WP 3, we can create a dependency relationship map that illustrates how different components are interconnected. This map resembles a genetic lineage chart, showing the relationships between genes or, in this case, dependencies. It reveals which parts of the code rely on others, just as a genetic lineage chart displays how traits or genes are passed down through generations.

Given a new project, we conduct in-depth analysis of the dependencies to assess their characteristics, including their functionality, stability, and versioning. This analysis is akin to evaluating the genetic traits or attributes inherited from ancestors. For instance, we assess whether a specific dependency exhibits desirable traits like stability or compatibility with the project. Then, we can examine how dependencies are inherited and utilized within the software project. Specifically, we create a comprehensive lineage chart that depicts how dependencies are inherited within the software project and understand the parent-child relationships between components, which is akin to tracking genetic inheritance from one generation to the next. Based on the lineage chart, we can identify the paths of inheritance, noting how specific dependencies are passed down to different parts of the project. In this way, we can recognize the dependencies that serve as ancestors, passing on their characteristics to descendant components. Also, we assess how the inheritance of dependencies affects the project's overall performance and behavior. This includes evaluating whether the inheritance of certain dependencies leads to enhanced functionality or potential issues. Considering the positive and negative impacts of inheritance, similar to assessing the impact of inherited genetic traits. During software traceability analysis, we will maintain detailed records including the attributes of each dependency, the name, version, functionality, and any identified issues. This documentation serves as a genetic trace archive, providing a historical record of dependency characteristics and their impact on the project.

By conducting these detailed steps in "Genetic Traceability" using dependency analysis, we can gain a deep understanding of how dependencies inherit traits and attributes, influence functionality and performance, and impact the overall genetic health of our software project. This approach contributes to effective management, optimization, and evolution of software components, ensuring that the project remains robust and reliable over time.


\subsubsection{Diagnostic Testing → SCA-Vulnerability Analysis}

Diagnostic testing in the context of software vulnerability analysis is akin to a comprehensive health checkup for software. It involves a detailed examination of each identified vulnerability within its respective software component. 

Before conducting vulnerability analysis, we first integrate our vulnerability genomics into the analysis framework. This dataset serves as the reference "genetic code" against which we'll compare our project's software components. It contains information about known vulnerabilities and weaknesses in various software components. Vulnerability analysis is an intricately detailed and multifaceted process. It initiates with an exhaustive code review conducted by seasoned software experts. This review encompasses a granular examination of the source code linked to each identified vulnerability. The objective is to dissect the code's structure, logic, and the precise location of vulnerabilities. In parallel, an equally thorough analysis of configuration settings is undertaken, with a focus on detecting potential vulnerabilities rooted in misconfigurations, improper settings, or configurations that might expose vulnerabilities. Dependencies, including third-party libraries and modules, undergo comprehensive scrutiny to ensure that vulnerabilities originating from these dependencies are not overlooked.

The diagnostic testing process extends to practical testing, where controlled experiments are conducted to assess the real-world exploitability of vulnerabilities. This practical assessment provides valuable insights into the likelihood of vulnerabilities being successfully exploited by malicious actors. Simultaneously, an impact assessment evaluates not only the technical aspects of each vulnerability but also its broader consequences. This includes assessing potential data breaches, system compromises, or service interruptions resulting from vulnerability exploitation. The diagnostic testing phase culminates in the development of highly tailored remediation recommendations. These recommendations vary from precise code modifications to critical configuration adjustments and updates to dependencies. 

Throughout the entire process, meticulous records are maintained, creating a comprehensive reference for the software's security history. This level of diagnostic testing leaves no facet of a vulnerability unexamined, ensuring a profound understanding of each vulnerability, which, in turn, leads to the most effective treatment and the creation of an enduring record documenting the software's "genetic health."

\subsection{Software Maintenance}
The objective of this WP is from another angle to translate the insights gained from our software genome analysis into practical real-world applications. In this WP, we simulate genetic engineering and develop predictive models to enhance software maintenance from two different perspectives (i.e., software patching and software optimization).

\subsubsection{Gene Therapy → Software Patching}

Given the excessive usage of third-party artifacts in contemporary software development, existing software also suffer from the potential threats from untrustworthy third-party artifacts (i.e., the various defective software genes unveiled in WP2). Although maintaining a comprehensive open-source intelligence platform can extensively trigger alarms when potential threats occur, tons of such alarms could also easily frustrate maintainers by significant manual works of mitigation. Moreover, conflicts or even new threats could also be brought when conducting threat mitigations. 

The objective of this task is to systematically tackle the potential threats of the defective software genes pinpointed by our open-source intelligence platform, with the most beneficial holistic outcome. Specifically, three pivotal research aims are going to be tackled: 1) Holistic threat mitigation approaches. Typically, there are three major solutions for handling potential threats, adopting patches, altering component versions, and replacing artifacts, the first two are common in modern vulnerability remediation solutions, while it is crucial to appropriately combining these three solutions to mitigate various software threats as we unveiled in WP2. 2) Contextual mitigation prioritization. Considering that not all identified software threats bring equal risks, our subsequent thrust is towards devising a context-aware prioritization mechanism. This ensures that the gravest threats are tackled with the urgency they warrant. For example, security vulnerabilities should be differently handled as they are usually only able to be triggered with different conditions, and the potential risks they could cause also significantly vary. Therefore, properly prioritizing vulnerabilities with mandatory requirements of mitigation could greatly save maintainers’ efforts. 3) Safeguarding against secondary hazards. The journey of threat mitigation is not devoid of potential pitfalls. Rectifying one potential threat could inadvertently introduce new issues, including but not limited to introducing new security threats, introducing artifacts with poor maintenance and code quality, violating software license compatibility, etc. Therefore, during the automated mitigation of defective software threats, we aim to proactively circumvent these secondary challenges, assuring a seamless, comprehensive resolution.

The remediation of threats of software defective genes is designed to bridge the gap between identified potential threats within the supply chain of software and the properly mitigation the threats that really threaten user projects. Based on this, software maintainers could be rescued from tons of alarms of defective software threats and concentrate on tackling those that really matter. Based on this, the lifecycle of defective software genes is closed on the open-source intelligence platform.


\subsubsection{Transgenic Technology → Software Refactoring}

Apart from security threats, Software optimization has become a paramount concern in the fast-evolving technological landscape. Insights and practices gleaned from the open-source ecosystem offer valuable benchmarks for enhancing performance, security, and efficiency in software development. OSS, characterized by its collaborative nature, transparency, and diversity, provides a rich repository of methodologies, tools, and techniques that have been tested and refined through collective input from a global community of developers. The application of practices learned from OSS not only accelerates innovation but also ensures that software products are robust, scalable, and aligned with the emerging trends and standards. In this context, the integration of OSS insights is instrumental in driving optimal software performance, adaptability, and user satisfaction.

This task aims to analyse existing user practices on optimizing open-source software and summarize best practices and generate recommendations for the maintenance and refactoring of open-source software. Specifically, we focus on, but not limited to the following aspects on optimizing software. 1) Bug fixing: apart from vulnerabilities, such as CVEs, that are known to the public, the numerous records of repository activities also undermine the millions of processing of potential software bugs, we aim to identify these bugs and their corresponding fixing commits, and based on which, summarizing the practices developers usually follow to mitigate the influence of bugs. 2) Architecture refactoring: as the continuous development of open-source software, technical debts, especially debts on software architecture, could gradually influence the stability and sustainability of software. While existing open-source repositories, such as GitHub and GitLab, record the most maintenance histories of open-source software. In this case, we aim to identify the practical operations of how open-source maintainers maintain the architecture of their software, such as the practices on implementing new functionalities and refactoring architectures when necessary. 3) Performance improvement: By meticulously analysing the development practices, one can extract actionable insights related to efficient memory usage, optimized CPU utilization, reduced latency, and enhanced throughput. Such insights may include patterns of code that make effective use of data structures, algorithms that optimize computational efficiency, or architectural designs that enhance scalability. These extracted practices, when applied, can significantly enhance the performance metrics of software, leading to faster execution times, reduced resource consumption, and an overall enhanced user experience.

Software optimization based on mining development practices could be treated as a more generalized mitigation of software defects, which is beyond the security threats we perform on Task 5.1. Moreover, such software optimizations could significantly ensure the quality of software and, consequently, preventing software defects from turning into real threats.


\subsection{Open Source Governance}
The objective of this WP is to establish robust open source governance. Drawing upon the comprehensive analysis outcomes of WP 1 through WP 5, our primary goal is to operationalize a suite of pivotal initiatives that encompass real-time intelligence prewarning, secured package manager, compatible semantic versioning, and license compliance. These initiatives collectively constitute the foundation upon which a well-structured and strategically governed open source ecosystem will be built.

\subsubsection{Real-time Intelligence Prewarning}
Given the dynamic and expansive nature of the open-source ecosystem, vulnerabilities, security threats, and other challenges can emerge rapidly, necessitating real-time responses. With an increasing number of contributors and a vast array of projects evolving simultaneously, the potential for overlooked bugs, security breaches, and the rapid propagation of vulnerabilities is heightened. Moreover, the collaborative and open-ended nature of open-source development sometimes leads to unintended security lapses and quality inconsistencies. Therefore, adopting a comprehensive intelligence monitoring system empowers stakeholders to track, analyse, and respond to various issues proactively. This proactive stance ensures that remedial actions, updates, or patches can be deployed expediently, safeguarding the integrity, security, and performance of open-source software while bolstering the overall resilience of the open-source ecosystem.

Our overarching objective compasses the real-time scanning of repositories, analysing code modifications, and monitoring discussion forums and contribution patterns to identify potential threats or areas of concern. Prewarning systems, embedded within this intelligence framework, are designed to alert developers, users, and administrators of emerging vulnerabilities or erratic behavioural patterns in real-time. This framework by leveraging a curated repository of open-source software and a meticulously designed security intelligence system. This framework is poised to deliver swift and precise services for the identification of software security threats, and offer an innovative solution that facilitates the fast and precise detection of the influence of these security threats. Through the integration of these essential elements, we envision a dynamic toolset that not only enhances the efficiency of software analysis but also contributes to the fortification of software ecosystems against potential risks and threats.

\emph{Lightweight and Fast SCA.}
It is non-trivial to identify the existence of security threats within open-source repositories and components. We first propose efficient and effective solutions on recognizing the impact of security threats. First, for source-code level analysis, we propose precise POM-based and code-clone-based solutions on light-weighted SCA to enhance performance, while for binary level analysis, prevailing methods often rely on intricate program analysis to reverse engineer binary code, extracting control flow graphs of functions and subsequently matching them to identify components. Regrettably, this approach proves exceedingly time-intensive, requiring hours for the analysis of a single binary. Given the scale of complex systems encompassing thousands of files, such an approach's viability diminishes. A further challenge arises from the lack of extracted features from program analysis, impeding accurate detection using syntactic attributes. To surmount these challenges, we propose a two-fold solution. Firstly, we curate the collected open-source dataset through meticulous duplicate removal, mitigating noise stemming from internal dependencies. Secondly, we extract strings from these projects, serving as lightweight features. By clustering these strings according to macros defined within the project source code, we exploit the likelihood of co-occurrence in compiled binaries. Employing an adaptive rating system, we gauge an open-source project's applicability based on string cluster matching percentages. Our approach aims to achieve precise SCA results while upholding commendable performance levels, especially when assessing substantial projects.

\emph{Security Threat Prediction and Confirmation.}
Following the completion of SCA, a comprehensive bill of materials for the analyzed projects is acquired. This serves as the foundation for the subsequent critical phase: identifying security threats associated with the open-source packages. This complex task is accomplished by harnessing the security threats database, allowing for the establishment of a robust linkage between security threats and their corresponding projects. To further enhance the precision of this process and reduce false positives, a multi-pronged approach is employed. Firstly, a set of pipelines will be designed to monitor the intelligence of open source security threats, based on which, new reports and news of software defects will be properly captured and processed. Next, program analysis is leveraged in conjunction with the capabilities of a sophisticated large language model (LLM) that comprehends the semantics of potentially vulnerable function candidates. At the binary level, functional features are extracted to predict the collective purpose of groups of binary instructions. Based on this purpose, the LLM extracts high-level abstractions of the functions' behaviors, facilitating a nuanced assessment of their integrity. Particularly, the system determines whether any malicious intent is present. In instances where malicious behavior is identified, the vulnerability is subsequently confirmed, and a comprehensive elucidation of the underlying cause is provided. This multifaceted approach not only ensures a meticulous detection of vulnerabilities but also offers insights into the intricacies of the identified security concerns.

\subsubsection{Secured Package Manager}

With the excessive reuse of existing third-party artifacts from public repositories, various threats could be introduced via software supply chain, by means of both dependency imports and code fragment reuse. In this case, this task aims to establish a set of infrastructure of secured package manager to secure the reuse of third-party artifacts for downstream users.

Specifically, the secured package manager includes six major components: 1) Secured Registry, serves as a three-layer artifact registry for hosting reusable artifacts, including patched registry for artifacts with known defects, audited registry for monitoring commonly used artifacts, and public registry for access to public repositories. 2) Secured Advisory, serves as an advisory database to record all the defective genes of open-source artifacts in WP2, based on which, open-source intelligence could be fully used to monitor the supply chain of user applications. 3) Client, is the client for users to manipulate their dependencies on third party artifacts, with which, users can not only manage their dependencies in secured way but also conduct necessary checking before publishing. 4) Backend Engine, is the server-side engine that optimizes the reuse of third-party artifacts from user clients, including prioritizing the dependency resolution by avoid open-source defects and controlling artifacts publishing and withdrawing. 5) Auditing Engine, serves as a cluster of engines that provide the ability to analyse open-source artifacts, based on which, a comprehensive profile of user required artifacts could be generated to guide user behaviours (i.e., publishing, withdrawing, and importing, etc.). 6) Configuration Language, serves as a set of domain specific language for configuring the reuse of third-party artifacts, not only for existing packages, but also for the commonly reused code fragments. With this, users are allowed to configure their requirements of dependencies in a more light-weighted and flexible way, including the thresholds and preferences during the resolution and remediation of dependencies. 

The secured package manager is specifically designed to provide a more secured and light-weighted solution for the publishment, maintenance, distribution, integration of the reuse of third-party artifacts for users. Based on this, the powerful open-source intelligence system of Software Genome could be easily utilized to user side, which also amplifies the ability of open source governance and surveillance.

\subsubsection{Compatible Semantic Versioning}

Open source software is usually maintained and released with certain agreement on its compatibility by following the semantic versioning, which plays a crucial role in software development, ensuring that updates and changes to software are systematically and clearly communicated to developers and end-users alike. Generally, it follows a structured format of version numbering and is essential for tracking software changes, managing dependencies, and maintaining system stability. However, in practice, inconsistencies and deviations in adhering to semantic versioning can lead to confusion, dependency errors, and system breakdowns. Therefore, the intricate landscape of software evolution, characterized by frequent updates and iterative enhancements, necessitates a stringent, standardized approach to adhere semantic versioning.

Therefore, this task aims to propose proper solutions to detecting violations and improving the adherence of software releases with semantic versioning. Specifically, we aim to achieve ecosystem-wide mitigation of incompatible releases by three steps. 1) Compatibility detection tool: existing researches focus on detecting software incompatible changes by check API signatures, and fail to detecting the impact of changes on intra-procedural functionalities that happen in the internal changes of API implementation, leaving behavioural incompatibilities undetectable. In this case, we first integrate compatibility detection with finer-grained behavioural change detection to enhance compatibility tools. 2) Compatible release check: from the perspective of library maintainers, we are able to tell whether an artifact to be released are compatible with previous releases based on our compatibility tool, and based on this, we set up pipelines to monitor the daily release in major ecosystems, and trigger warnings when incompatible non-major releases happen. 3) Compatible upgrades: from the perspective of users, dependency updates are non-trivial to downstream users for the purpose of including new features and fixing necessary bugs. However, conducting such dependency upgrades could introduce compatible issues that could compromise user software. We aim to propose corresponding tools to help users finding released versions that are compatible with their deployed ones and manage the dependency configurations with proper flexibility on dependency ranges.

This set of compatible semantic versioning tools aim to provide solutions on managing software dependencies in a flexible but compatible way, which could benefit the management of technical lags and software defect mitigation from the perspective of both upstream maintenance and downstream usage, developers and users can have clear, unambiguous insights into the changes embedded in each software release, fostering informed decision-making, seamless integration, and system stability.

\subsubsection{License Compliance}

Reusing code fragments or third-party libraries from existing repositories has significantly accelerated the modern software development, while it also places potential legal risks of violating license compatibility due to lack of legal expertise. In this case, as one of the most crucial defects, it is vital to properly examining and managing the usage of licensed artifacts, which could largely decrease the legal risks on reusing existing coding features in modern software development.
Our objective is to propose a complementary and comprehensive metamodel of software licenses, and based on it, collect and interpret licenses of existing code fragments, especially the code features in software genome, in a proper manner. Such an in-depth interpretation of software licenses could significantly enhance the risk management of license-related intelligence across the open-source ecosystem.

\emph{License Metamodel.}
First, starting with the well-known software licenses, such as SPDX licenses and FOSS licenses, we plan to conduct an in-depth analysis to interpret the rights and obligations defined in these popular software licenses. Specifically, though existing researches have labelled existing software licenses with terms of rights and obligations, they are still with coarse-grained interpretation which fail to capture more fine-grained requirements and scenarios. We aim to collect existing interpretations that are in different labelling system, and regulate them in a more standardized way by differential analysis. Apart from existing term classifications, we will also step forward to propose a comprehensive metamodel for more fine-grained license modelling. 

\emph{License Conflict Modelling.}
Next, we will also propose the license incompatibility model for code reuse based on our fine-grained license modelling. Specifically, there could be different types of license conflicts for different reasons. For instance, 1) Attitude conflicts. Reusing code fragments that are under restrictive licenses could be risky as obligations required could be easily ignored by project licenses (especially permissive licenses), which could be easily neglected by maintainers. 2) Conditional Conflicts. Some licenses only grant specific rights under specific conditions, while these conditions could be neglected if only term-level conflicts are taken into consideration. 3) Copyleft Conflicts. Copyleft licenses naturally require the granted rights to be inherited by downstream users of licensed code fragments, otherwise illegality could be introduced in downstream user projects. In this case, based on the license metamodel, we will further conclude a complementary and comprehensive license conflict model to guide further risk management on license compatibility.

\emph{Customized License Identification.}
Moreover, besides popular software licenses, there are still massive customized software licenses in the open source ecosystem. In this case, based on the license modelling, we aim to empower the ability of recognizing the diverse customized licenses and interpret them into our metamodel. Specifically, starting with the license texts of existing well-interpreted licenses, we feed them, as well as the structured modelling of these licenses, into large language models (LLMs) to guide the classification of licenses. We aim to reuse the ability of LLMs on interpreting license texts and guide them to modelling these licenses based on our own license metamodel. Based on this, we are able to automate the interpretation of the massive customized licenses and convert them into a structured model, with which, further incompatibility analysis could be further conducted, and more fine-grained risk management could be properly carried out.

